Producing 3D Friction Loads by Tracking the Motion of the Contact Point on Bodies in Mutual Contact

We outline a phenomenological model to assess friction at the interface between two bodies in mutual contact. Although the approach is general, the application inspiring the approach is the Discrete Element Method. The kinematics of the friction process is expressed in terms of the relative 3D motion of the contact point on the two surfaces in mutual contact. The model produces expressions for three friction loads: slide force, roll torque, and spin torque. The cornerstone of the methodology is the process of tracking the evolution/path of the contact point on the surface of the two bodies in mutual contact. The salient attribute of the model lies with its ability to simultaneously compute, in a 3D setup, the slide, roll, and spin friction loads for smooth bodies of arbitrary geometry while accounting for both static and kinematic friction coefficients.

==> macros.tex <==
\graphicspath{{Images/}}
\newcommand{\CHRONO}{{\sffamily{{Chrono}}}}
\newcommand{\support}[1]{{{\mathcal{S}({#1})}}}
\newcommand{\SBELfeedbackONE}[1]{{\bf{\textcolor{red}{#1}}}} 
\newcommand{\SBELfeedbackTWO}[2]{{\bf{\textcolor{red}{#1}}} {\textcolor{blue}{(#2)}}}
\newcommand{\body}[1]{{b_{#1}}}
\newcommand{\tngPlane}[1]{{\tau_{#1}}}
\newcommand{\cPoint}[2]{{C_{#1}^{#2}}}
\newcommand{\prjCPoint}[2]{{{\bar C}_{#1}^{#2}}}
\newcommand{\nAxis}[1]{{\bf n}_{#1}}
\newcommand{\uAxis}[1]{{\bf u}_{#1}}
\newcommand{\wAxis}[1]{{\bf w}_{#1}}
\newcommand{\nAxTwo}[2]{{\bf n}_{#1}^{#2}}
\newcommand{\uAxTwo}[2]{{\bf u}_{#1}^{#2}}
\newcommand{\wAxTwo}[2]{{\bf w}_{#1}^{#2}}
\newcommand{\uBarAxis}[1]{{\bar{\bf u}}_{#1}}
\newcommand{\wBarAxis}[1]{{\bar{\bf w}}_{#1}}
\newcommand{\dirArc}[1]{{\vec{s}}_{#1}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\EVal}{{\bf S}_{ij}}
\newcommand{\dltaEVal}{{\Delta{\bf S}_{ij}}}
\newcommand{\EValSize}{\|{\bf S}_{ij}\|}
\newcommand{\SlideFForceE}{{\bf E}_{f}}
\newcommand{\SlideFForceD}{{\bf D}_{f}}
\newcommand{\SlideFForce}{{\bf F}_{f}}
\newcommand{\CurvRoll}{{\kappa}}
\newcommand{\RollFricTorque}{{\bm{\mathcal{T}}}}
\newcommand{\SlackSsTh}{{\mathcal{S}_s^S}}
\newcommand{\SlackSkTh}{{\mathcal{S}_k^S}}
\newcommand{\SlackS}{{\mathcal{S}^S}}
\newcommand{\SlackRsTh}{{\mathcal{S}_s^R}}
\newcommand{\SlackRkTh}{{\mathcal{S}_k^R}}
\newcommand{\SlackR}{{\mathcal{S}^R}}
\newcommand{\SlackPsisTh}{{\mathcal{S}_s^\psi}}
\newcommand{\SlackPsikTh}{{\mathcal{S}_k^\psi}}
\newcommand{\SlackPsi}{{\mathcal{S}^\psi}}
\newcommand{\SlideFunction}[2]{{\mathcal{F}^\psi_{#1}({#2})}}
\newcommand{\SpinFunction}[2]{{\mathcal{F}^\psi_{#1}({#2})}}
\newcommand{\SpinFunctionDamping}[1]{{\mathcal{F}^\psi_D({#1})}}
\newcommand{\SpinFricTorque}{{\mathcal{T}}^\psi}
\newcommand{\SpinFricTorqueE}{{\mathcal{T}}^\psi_E}
\newcommand{\SpinFricTorqueD}{{\mathcal{T}}^\psi_D}



